A Restricted Black-box Adversarial Framework Towards Attacking Graph Embedding Models

With the great success of graph embedding model on both academic and industry area, the robustness of graph embedding against adversarial attack inevitably becomes a central problem in graph learning domain. Regardless of the fruitful progress, most of the current works perform the attack in a white-box fashion: they need to access the model predictions and labels to construct their adversarial loss. However, the inaccessibility of model predictions in real systems makes the white-box attack impractical to real graph learning system. This paper promotes current frameworks in a more general and flexible sense -- we demand to attack various kinds of graph embedding model with black-box driven. To this end, we begin by investigating the theoretical connections between graph signal processing and graph embedding models in a principled way and formulate the graph embedding model as a general graph signal process with corresponding graph filter. As such, a generalized adversarial attacker: GF-Attack is constructed by the graph filter and feature matrix. Instead of accessing any knowledge of the target classifiers used in graph embedding, GF-Attack performs the attack only on the graph filter in a black-box attack fashion. To validate the generalization of GF-Attack, we construct the attacker on four popular graph embedding models. Extensive experimental results validate the effectiveness of our attacker on several benchmark datasets. Particularly by using our attack, even small graph perturbations like one-edge flip is able to consistently make a strong attack in performance to different graph embedding models.

==> GF_Attack <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{{Akhtar} and {Mian}}{2018}]{akhtar2018threat}
{Akhtar}, N., and {Mian}, A.~S.
\newblock 2018.
\newblock Threat of adversarial attacks on deep learning in computer vision: A
  survey.
\newblock {\em IEEE Access} 6:14410--14430.

\bibitem[\protect\citeauthoryear{Bojchevski and
  G{\"u}nnemann}{2019}]{icml2019adversarial}
Bojchevski, A., and G{\"u}nnemann, S.
\newblock 2019.
\newblock Adversarial attacks on node embeddings via graph poisoning.
\newblock In {\em International Conference on Machine Learning},  695--704.

\bibitem[\protect\citeauthoryear{Cui \bgroup et al\mbox.\egroup
  }{2018}]{cui2018survey}
Cui, P.; Wang, X.; Pei, J.; and Zhu, W.
\newblock 2018.
\newblock A survey on network embedding.
\newblock {\em IEEE Transactions on Knowledge and Data Engineering}
  31(5):833--852.

\bibitem[\protect\citeauthoryear{{Dai} \bgroup et al\mbox.\egroup
  }{2018}]{ICML2018Adversarial}
{Dai}, H.; {Li}, H.; {Tian}, T.; {Huang}, X.; {Wang}, L.; {Zhu}, J.; and
  {Song}, L.
\newblock 2018.
\newblock Adversarial attack on graph structured data.
\newblock {\em international conference on machine learning}  1115--1124.

\bibitem[\protect\citeauthoryear{{Defferrard}, {Bresson}, and
  {Vandergheynst}}{2016}]{Defferrard2016ChebNet}
{Defferrard}, M.; {Bresson}, X.; and {Vandergheynst}, P.
\newblock 2016.
\newblock Convolutional neural networks on graphs with fast localized spectral
  filtering.
\newblock {\em neural information processing systems}  3844--3852.

\bibitem[\protect\citeauthoryear{{Duvenaud} \bgroup et al\mbox.\egroup
  }{2015}]{duvenaud2015convolutional}
{Duvenaud}, D.~K.; {Maclaurin}, D.; {Aguilera-Iparraguirre}, J.;
  {Gómez-Bombarelli}, R.; {Hirzel}, T.; {Aspuru-Guzik}, A.; and {Adams}, R.~P.
\newblock 2015.
\newblock Convolutional networks on graphs for learning molecular fingerprints.
\newblock {\em neural information processing systems}  2224--2232.

\bibitem[\protect\citeauthoryear{{Hamilton}, {Ying}, and
  {Leskovec}}{2017}]{Hamilton2017Inductive}
{Hamilton}, W.~L.; {Ying}, Z.; and {Leskovec}, J.
\newblock 2017.
\newblock Inductive representation learning on large graphs.
\newblock {\em neural information processing systems}  1024--1034.

\bibitem[\protect\citeauthoryear{{Kipf} and {Welling}}{2017}]{ICLR2017SemiGCN}
{Kipf}, T.~N., and {Welling}, M.
\newblock 2017.
\newblock Semi-supervised classification with graph convolutional networks.
\newblock {\em international conference on learning representations}.

\bibitem[\protect\citeauthoryear{{McCallum} \bgroup et al\mbox.\egroup
  }{2000}]{Dataset2000Cora}
{McCallum}, A.~K.; {Nigam}, K.; {Rennie}, J.; and {Seymore}, K.
\newblock 2000.
\newblock Automating the construction of internet portals with machine
  learning.
\newblock {\em Information Retrieval} 3(2):127--163.

\bibitem[\protect\citeauthoryear{Nar \bgroup et al\mbox.\egroup
  }{2019}]{nar2019cross}
Nar, K.; Ocal, O.; Sastry, S.~S.; and Ramchandran, K.
\newblock 2019.
\newblock Cross-entropy loss and low-rank features have responsibility for
  adversarial examples.
\newblock {\em arXiv preprint arXiv:1901.08360}.

\bibitem[\protect\citeauthoryear{Ortega \bgroup et al\mbox.\egroup
  }{2018}]{ortega2018graph}
Ortega, A.; Frossard, P.; Kova{\v{c}}evi{\'c}, J.; Moura, J.~M.; and
  Vandergheynst, P.
\newblock 2018.
\newblock Graph signal processing: Overview, challenges, and applications.
\newblock {\em Proceedings of the IEEE} 106(5):808--828.

\bibitem[\protect\citeauthoryear{{Paranjape}, {Benson}, and
  {Leskovec}}{2017}]{paranjape2017motifs}
{Paranjape}, A.; {Benson}, A.~R.; and {Leskovec}, J.
\newblock 2017.
\newblock Motifs in temporal networks.
\newblock In {\em Proceedings of the Tenth ACM International Conference on Web
  Search and Data Mining},  601--610.

\bibitem[\protect\citeauthoryear{Perozzi, Al-Rfou, and
  Skiena}{2014}]{perozzi2014deepwalk}
Perozzi, B.; Al-Rfou, R.; and Skiena, S.
\newblock 2014.
\newblock Deepwalk: Online learning of social representations.
\newblock In {\em Proceedings of the 20th ACM SIGKDD international conference
  on Knowledge discovery and data mining},  701--710.
\newblock ACM.

\bibitem[\protect\citeauthoryear{{Qiu} \bgroup et al\mbox.\egroup
  }{2018}]{WSDM2018NetworkEmbedding}
{Qiu}, J.; {Dong}, Y.; {Ma}, H.; {Li}, J.; {Wang}, K.; and {Tang}, J.
\newblock 2018.
\newblock Network embedding as matrix factorization: Unifying deepwalk, line,
  pte, and node2vec.
\newblock In {\em Proceedings of the Eleventh ACM International Conference on
  Web Search and Data Mining},  459--467.

\bibitem[\protect\citeauthoryear{{Scarselli} \bgroup et al\mbox.\egroup
  }{2009}]{scarselli2009GNN}
{Scarselli}, F.; {Gori}, M.; {Tsoi}, A.~C.; {Hagenbuchner}, M.; and
  {Monfardini}, G.
\newblock 2009.
\newblock The graph neural network model.
\newblock {\em IEEE Transactions on Neural Networks} 20(1):61--80.

\bibitem[\protect\citeauthoryear{{Sen} \bgroup et al\mbox.\egroup
  }{2008}]{Dataset2008Citeseer}
{Sen}, P.; {Namata}, G.~M.; {Bilgic}, M.; {Getoor}, L.; {Gallagher}, B.; and
  {Eliassi-Rad}, T.
\newblock 2008.
\newblock Collective classification in network data.
\newblock {\em Ai Magazine} 29(3):93--106.

\bibitem[\protect\citeauthoryear{{Shuman} \bgroup et al\mbox.\egroup
  }{2013}]{shuman2013GSP}
{Shuman}, D.~I.; {Narang}, S.~K.; {Frossard}, P.; {Ortega}, A.; and
  {Vandergheynst}, P.
\newblock 2013.
\newblock The emerging field of signal processing on graphs: Extending
  high-dimensional data analysis to networks and other irregular domains.
\newblock {\em IEEE Signal Processing Magazine} 30(3):83--98.

\bibitem[\protect\citeauthoryear{{Sun} \bgroup et al\mbox.\egroup
  }{2018}]{sun2018adversarial}
{Sun}, L.; {Wang}, J.; {Yu}, P.~S.; and {Li}, B.
\newblock 2018.
\newblock Adversarial attack and defense on graph data: A survey.
\newblock {\em arXiv preprint arXiv:1812.10528}.

\bibitem[\protect\citeauthoryear{{Tang} \bgroup et al\mbox.\egroup
  }{2015}]{WWW2015Line}
{Tang}, J.; {Qu}, M.; {Wang}, M.; {Zhang}, M.; {Yan}, J.; and {Mei}, Q.
\newblock 2015.
\newblock Line: Large-scale information network embedding.
\newblock In {\em Proceedings of the 24th International Conference on World
  Wide Web},  1067--1077.

\bibitem[\protect\citeauthoryear{{Tong} \bgroup et al\mbox.\egroup
  }{2012}]{CIKM2012Gelling}
{Tong}, H.; {Prakash}, B.~A.; {Eliassi-Rad}, T.; {Faloutsos}, M.; and
  {Faloutsos}, C.
\newblock 2012.
\newblock Gelling, and melting, large graphs by edge manipulation.
\newblock In {\em Proceedings of the 21st ACM international conference on
  Information and knowledge management},  245--254.

\bibitem[\protect\citeauthoryear{Tu \bgroup et al\mbox.\egroup
  }{2018}]{tu2018deep}
Tu, K.; Cui, P.; Wang, X.; Yu, P.~S.; and Zhu, W.
\newblock 2018.
\newblock Deep recursive network embedding with regular equivalence.
\newblock In {\em Proceedings of the 24th ACM SIGKDD International Conference
  on Knowledge Discovery \& Data Mining},  2357--2366.
\newblock ACM.

\bibitem[\protect\citeauthoryear{Wu \bgroup et al\mbox.\egroup
  }{2019}]{sgc_icml19}
Wu, F.; Zhang, T.; Souza~Jr., A.~H.; Fifty, C.; Yu, T.; and Weinberger, K.~Q.
\newblock 2019.
\newblock Simplifying graph convolutional networks.
\newblock In {\em Proceedings of the 36th International Conference on Machine
  Learning (ICML)}.

\bibitem[\protect\citeauthoryear{{Xu} \bgroup et al\mbox.\egroup
  }{2018}]{xu2018how}
{Xu}, K.; {Hu}, W.; {Leskovec}, J.; and {Jegelka}, S.
\newblock 2018.
\newblock How powerful are graph neural networks.
\newblock {\em arXiv preprint arXiv:1810.00826}.

\bibitem[\protect\citeauthoryear{{Xu} \bgroup et al\mbox.\egroup
  }{2019}]{xu2019topology}
{Xu}, K.; {Chen}, H.; {Liu}, S.; {Chen}, P.-Y.; {Weng}, T.-W.; {Hong}, M.; and
  {Lin}, X.
\newblock 2019.
\newblock Topology attack and defense for graph neural networks: An
  optimization perspective.
\newblock {\em arXiv preprint arXiv:1906.04214}.

\bibitem[\protect\citeauthoryear{{Yang} and {Liu}}{2015}]{yang2015Comprehend}
{Yang}, C., and {Liu}, Z.
\newblock 2015.
\newblock Comprehend deepwalk as matrix factorization.
\newblock {\em arXiv preprint arXiv:1501.00358}.

\bibitem[\protect\citeauthoryear{Yang \bgroup et al\mbox.\egroup
  }{2015}]{yang2015network}
Yang, C.; Liu, Z.; Zhao, D.; Sun, M.; and Chang, E.
\newblock 2015.
\newblock Network representation learning with rich text information.
\newblock In {\em Twenty-Fourth International Joint Conference on Artificial
  Intelligence}.

\bibitem[\protect\citeauthoryear{{Zhu} \bgroup et al\mbox.\egroup
  }{2018}]{zhu2018high}
{Zhu}, D.; {Cui}, P.; {Zhang}, Z.; {Pei}, J.; and {Zhu}, W.
\newblock 2018.
\newblock High-order proximity preserved embedding for dynamic networks.
\newblock {\em IEEE Transactions on Knowledge and Data Engineering}
  30:2134--2144.

\bibitem[\protect\citeauthoryear{{Zügner}, {Akbarnejad}, and
  {Günnemann}}{2018}]{KDD2018Adversarial}
{Zügner}, D.; {Akbarnejad}, A.; and {Günnemann}, S.
\newblock 2018.
\newblock Adversarial attacks on neural networks for graph data.
\newblock In {\em Proceedings of the 24th ACM SIGKDD International Conference
  on Knowledge Discovery \& Data Mining},  2847--2856.

\bibitem[\protect\citeauthoryear{{Zügner} and
  {Günnemann}}{2019}]{ICLR2019Meta}
{Zügner}, D., and {Günnemann}, S.
\newblock 2019.
\newblock Adversarial attacks on graph neural networks via meta learning.
\newblock {\em international conference on learning representations}.

\end{thebibliography}

